TextAdaIN: Paying Attention to Shortcut Learning in Text Recognizers

Leveraging the characteristics of convolutional layers, neural networks are extremely effective for pattern recognition tasks. However in some cases, their decisions are based on unintended information leading to high performance on standard benchmarks but also to a lack of generalization to challenging testing conditions and unintuitive failures. Recent work has termed this "shortcut learning" and addressed its presence in multiple domains. In text recognition, we reveal another such shortcut, whereby recognizers overly depend on local image statistics. Motivated by this, we suggest an approach to regulate the reliance on local statistics that improves text recognition performance. Our method, termed TextAdaIN, creates local distortions in the feature map which prevent the network from overfitting to local statistics. It does so by viewing each feature map as a sequence of elements and deliberately mismatching fine-grained feature statistics between elements in a mini-batch. Despite TextAdaIN's simplicity, extensive experiments show its effectiveness compared to other, more complicated methods. TextAdaIN achieves state-of-the-art results on standard handwritten text recognition benchmarks. It generalizes to multiple architectures and to the domain of scene text recognition. Furthermore, we demonstrate that integrating TextAdaIN improves robustness towards more challenging testing conditions. The official Pytorch implementation can be found at https://github.com/amazon-research/textadain-robust-recognition.

==> tables/SpAdaIN_breakdown_transposed.tex <==
\begin{table}
\normalsize
\begin{center}
\small
\bgroup
% \def\arraystretch{1.1}
    \begin{tabular}{c| c | c | c c c c c | c c c c c | c} 
      \toprule
      \multicolumn{1}{c}{} & \multicolumn{1}{c}{Baseline} &
      \multicolumn{1}{c}{AdaIN} &
      \multicolumn{10}{c}{AdaIN Variations} & \multicolumn{1}{c}{\AlgoName} \\ 
      \midrule
      AdaIN Dim & - & C & W & H & H, W & C, W & C, H & C & W & H & H, W & C, W & C, H \\
    %   \midrule
      Windows & - & - & - & - & - & - & - & 5 & 5 & 5 & 5 & 5 & 5 \\      
    %   \midrule
      IAM Accuracy & 85.7 & 85.4 & 85.7 & 85.6 & 85.7 & 85.8 & 85.9 & 85.9 & 85.5 & 85.9 & 85.8 & 85.9 & \textbf{87.3} \\
      \bottomrule
      
    \end{tabular}
\egroup
\tiny
\caption{\textbf{AdaIN dimensions.} Accuracy on the IAM dataset when applying the AdaIN operation over different dimensions. Our method, \AlgoNameNoSpace, shows significant improvement upon the baseline of \textbf{+1.6} pp. }
% \label{tab:spAdaIN_configuration}
\vspace{-0.8cm}
\end{center}
\end{table}

==> tables/padain_vs_spadain_transposed.tex <==
\begin{table}
\normalsize
\begin{center}
\small
\caption{\textbf{Probability of applying \AlgoNameNoSpace.} Applying AdaIN at high values of $p$ has little effect on the performance, demonstrating there is no shortcut learning in the form of global image statistic as in classification tasks \cite{nuriel2021permuted}. In contrast, profusely applying \AlgoName distorts important information that the model relies on. Therefore, with the right $p$, \AlgoName can moderate the reliance on local statistics}
\bgroup
% \centering
%   \begin{center}
    \small
    \begin{tabular}{l | >{\centering\arraybackslash}p{1.5cm} | p{0.7cm} p{0.7cm} p{0.7cm} | p{0.7cm} p{0.7cm}  p{0.7cm} p{0.7cm} p{0.7cm} }
      \toprule
      \multicolumn{1}{l}{} & \multicolumn{1}{c}{\textbf{Baseline}} & \multicolumn{3}{c}{\textbf{AdaIN}} & \multicolumn{5}{c}{\textbf{\AlgoName}} \\ 
      
      \midrule
      $p$ & -- & 0.01 & 0.1 & 0.25 & 0.001 & 0.01 & 0.05 & 0.1 & 0.25\\
      \midrule
      IAM Accuracy & 85.7 & 85.4 & 85.9 & 85.8 & 86.1 & \textbf{87.3} & 86.8 & 78.0 & 74.7\\
    \bottomrule
    \end{tabular}


\egroup
\tiny

\label{tab:spadain_vs_padain}
\vspace{-0.85cm}
\end{center}
\end{table}


==> tables/textadain_vs_noise_small.tex <==

% \small
\bgroup
\caption{\textbf{The importance of the induced distribution.} Best performance is achieved only when injecting distortions from an induced distribution namely, other text images}
\def\arraystretch{1.1}
        \begin{tabular}{l|c|c}
        \toprule
        Injection Method & Donors & Accuracy \\
        \midrule
        Baseline & X & 85.7\\
        
        \midrule
        \AlgoName & Gaussian Noise & 86.1 \\
        \AlgoName & Blank Image & 86.2 \\
        \midrule
        \AlgoName & Text Images & \textbf{87.3}\\
        \bottomrule
    \end{tabular}
\egroup
\tiny

\label{tab:textadain_vs_noise_small}
\vspace{-0.8cm}

